A HPC Co-Scheduler with Reinforcement Learning

Although High Performance Computing (HPC) users understand basic resource requirements such as the number of CPUs and memory limits, internal infrastructural utilization data is exclusively leveraged by cluster operators, who use it to configure batch schedulers. This task is challenging and increasingly complex due to ever larger cluster scales and heterogeneity of modern scientific workflows. As a result, HPC systems achieve low utilization with long job completion times (makespans). To tackle these challenges, we propose a co-scheduling algorithm based on an adaptive reinforcement learning algorithm, where application profiling is combined with cluster monitoring. The resulting cluster scheduler matches resource utilization to application performance in a fine-grained manner (i.e., operating system level). As opposed to nominal allocations, we apply decision trees to model applications' actual resource usage, which are used to estimate how much resource capacity from one allocation can be co-allocated to additional applications. Our algorithm learns from incorrect co-scheduling decisions and adapts from changing environment conditions, and evaluates when such changes cause resource contention that impacts quality of service metrics such as jobs slowdowns. We integrate our algorithm in an HPC resource manager that combines Slurm and Mesos for job scheduling and co-allocation, respectively. Our experimental evaluation performed in a dedicated cluster executing a mix of four real different scientific workflows demonstrates improvements on cluster utilization of up to 51% even in high load scenarios, with 55% average queue makespan reductions under low loads.

==> packages.tex <==
%\usepackage{blindtext}
%\usepackage{geometry}                		% See geometry.pdf to learn the layout options. There are lots.
%\geometry{letterpaper}                   		% ... or a4paper or a5paper or ... 
%\geometry{landscape}                		% Activate for rotated page geometry
%\usepackage[parfill]{parskip}    		% Activate to begin paragraphs with an empty line rather than an indent
\usepackage{graphicx}				% Use pdf, png, jpg, or eps§ with pdflatex; use eps in DVI mode
								% TeX will automatically convert eps --> pdf in pdflatex		
%\usepackage{amssymb}
\usepackage[misc]{ifsym}
%\usepackage{bbding}
\usepackage{svg}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\newcommand{\orcid}[1]{\href{https://orcid.org/#1}{\includesvg[width=10pt]{orcid}}}
%SetFonts
%\usepackage{savetrees }
%\usepackage[skip=0pt]{caption}
% cyb-sec.org

\newenvironment{tightItemize}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\usepackage[compact]{titlesec}
    \titlespacing{\section}{0pt}{2ex}{1ex}
    \titlespacing{\subsection}{0pt}{1ex}{0ex}
    \titlespacing{\subsubsection}{0pt}{0.5ex}{0.5ex}

\setlength{\textfloatsep}{30pt}
\setlength{\intextsep}{30pt}

\usepackage[colorinlistoftodos, textwidth=20mm, textsize=footnotesize]{todonotes}
  \newcommand{\abel}[1]{\todo[author=\textbf{Abel},color=orange!30,caption={},inline]{\emph{#1}}}
  \newcommand{\johan}[1]{\todo[author=\textbf{Johan},color=magenta!30,caption={},inline]{\emph{#1}}}
  \newcommand{\comm}[1]{\todo[author=\textbf{Comment},color=red!30,caption={},inline]{\emph{#1}}}
  
%\DeclareMathOperator*{\E}{\mathbb{E}}

\usepackage{cite}
\usepackage{url}
\usepackage{algorithmic}
%\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage[cmex10]{amsmath}
\usepackage{amssymb,amsmath}
\usepackage{psfrag,graphics,epsfig,epic,color,subfigure}
%\usepackage{graphicx} 
\usepackage{accents}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}

\newtheorem{Theorem}{Theorem}
\newtheorem{Corollary}{Corollary}
\newtheorem{Lemma}{Lemma}
\newtheorem{Proposition}{Proposition}
\newtheorem{Remark}{Remark}
\newtheorem{Definition}{Definition}
%\newenvironment{proof}{{\em Proof:} \ \ }{\begin{flushright}$\Box$\end{flushright}}

\newcommand{\bmat}[1]{ \begin{bmatrix} #1 \end{bmatrix} }
\newcommand{\R}{\mathbb{R}}

\newcommand{\AM}{\mathbf{A}}
\newcommand{\BM}{\mathbf{B}}
\newcommand{\CM}{\mathbf{C}}
\newcommand{\DM}{\mathbf{D}}
\newcommand{\FM}{\mathbf{F}}
\newcommand{\GM}{\mathbf{G}}
\newcommand{\IM}{\mathbf{I}}
\newcommand{\HM}{\mathbf{H}}
\newcommand{\KM}{\mathbf{K}}
\newcommand{\LM}{\mathbf{L}}
\newcommand{\MM}{\mathbf{M}}
\newcommand{\NM}{\mathbf{N}}
\newcommand{\OM}{\mathbf{O}}
\newcommand{\PM}{\mathbf{P}}
\newcommand{\QM}{\mathbf{Q}}
\newcommand{\RM}{\mathbf{R}}
\newcommand{\SM}{\mathbf{S}}
\newcommand{\TM}{\mathbf{T}}
\newcommand{\UM}{\mathbf{U}}
\newcommand{\VM}{\mathbf{V}}
\newcommand{\WM}{\mathbf{W}}
\newcommand{\XM}{\mathbf{X}}
\newcommand{\YM}{\mathbf{Y}}
\newcommand{\ZM}{\mathbf{Z}}
\newcommand{\SMM}{\mathbf{\Sigma}}

\newcommand{\av}{\mathbf{a}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\fv}{\mathbf{f}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\lv}{\mathbf{l}}
\newcommand{\mv}{\mathbf{m}}
\newcommand{\pv}{\mathbf{p}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\zv}{\mathbf{z}}

\newcommand{\N}{\mathbb{N}}
%\newcommand{\U}{\mathbb{U}}
%\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Model}{\mathcal{M}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\eye}{eye}
\DeclareMathOperator*{\trace}{tr}

==> sections/background_related.tex <==
\section{Related Work}

Reinforcement learning (RL) is defined as a problem with states, actions, and rewards, with state transitions which are affected by the current measured state, chosen action, and the environment. 
That is embedded in RL's definition, which is formulated as a Markov Decision Process. 
%Generally one will not find stateless variants of RL.
%However, there are related stateless problems. 
In multi-armed bandits, one just have actions and rewards. 
Solutions for multi-armed bandits allow for learning of reward based on actions, and can be optimised by selecting the best action.
Main optimisation problems are knowing the best action, and what total reward can be accumulated whilst still testing for which is the best action. 
Another common example might be advert selection online for anonymous visitors to a site. 
Although there is often plenty of data available, there is also a huge amount that is hidden, and a practical approach is to treat the probability of a click through as only depending on the choice of content, which is then the site's action.

There is a "stateful" variant of multi-armed bandits called contextual bandits - when there is some kind of signal that can be associated with the correct action, but actions taken have no effect on what the next state will be. Contextual bandits have states, actions and rewards, but no transition rules, they can be treated as a set of entirely separate events.

A contextual bandit with added transition rules between states, but no influence from the selected action, is essentially a sub-class of the reinforcement learning problem, and you can use most of the same analysis to predict long term reward and learn optimal behaviour.

And just for completeness, there are Markov Reward Processes without agent interaction that have states, and rewards, but no actions. It is possible to use reinforcement learning algorithms on these to predict long term reward and/or the expected long term value of being in a specific state.

In Bandit Scheduling Optimization \footnote{In classical multi-armed bandit problem formulation, a gambler is at a row of casino slot machines (in American-English slang, these are called "one-armed bandits") where she has to decide which machines to play at each time, how many times to play in  each machine and in which order to play them.}, one basically has a set of resources where jobs needs to be assigned according to an Object Function (OF).
This OF can be anything, like for example minimizing the average (expected) queue waiting time for submitted jobs.
The task one party (the learner, or player) has to do is to learn the probability distribution of each one of the available resources by interacting (exploring) with the system in a (finite) time interval during an experiment.
This interaction means, for instance, collocating two jobs in a resource. 
Then, after their execution ends, the learner observes the final status of each one of the jobs (often called 'Reward') . 
Metrics and questions can be posed by for example: "what constraints were or were not violated?", "How was the behavior evolution (CPU, memory, I/O, network,... over time) of the resources while both jobs were running together?".
This process can go for \textit{n} jobs in a pool of resources being managed by a specific queue in a Datacenter with a set of constraints, like for example, deadline.
Once enough learning (based on your questions) has been collected, the player starts exploiting the system in order to make better placements (collocation guesses) so a lower ratio of constraints are missed.

In Multi-Armed Bandit Optimization, there are usually two scenarios\footnote{There is a 3rd scenario, Markovian, but the techniques applied in their analysis are very different from what is done in Stochastic and Adversarial settings.}:\\
(i) Stochastic: The Probability Distributions from the resources you are learning about \textbf{does not} change over the time interval of an experiment;\\
(ii) Adversarial: The Probability Distributions from the resources you are learning about \textbf{does} maliciously (not too random) change over the time interval of an experiment, according to what one of the parties is doing;

An instance of a stochastic setting would be if one places two well behaved jobs in a same server for a couple of times and initiate them in the very same configuration for all repetitions.
There is a high probability that in the end the results will be the same.

On the other hand, in an adversarial setting, what happens is that the consequences of placing the very same jobs in the same server in each repetition would be different, since one of the jobs could (hypothetically) 'steal' resources by somehow learning the behavior of the other job in order to adapt to that.
The task of the learner (Job Scheduler) in this case is to try to learn this malicious behavior of the adversarial in order to mitigate the number of constraints missed.

There are different algorithms for giving theoretical bounds to how fast or how much one has to explore in order to fully learn the probability distributions for all resources. In both scenarios.
They differ in complexity of solution, time for convergence and others.

==> sections/old_IEEE_main.tex <==
\section{Introduction}


Low effective utilization of computation resources is a major drawback of many modern datacenters \cite{yang2013bubble}. 
In order to guarantee Quality-of-Services (QoS) and other requirements on the Service Level Agreements (SLAs) agreed with users, 
datacenter operators implement a worst-case view in resource allocation \cite{yang2013bubble}. 
Efficient resource allocation is however of direct interest to these operators
in case such theoretical guarantees can be provided.

This paper studies a more effective scheduling strategy for job placement which comes with strong theoretical guarantees.

\section{ASA and ASA$_{\mbox{X}}$}

Assume there are $m$ potentially good actions $\{a\}$, and that after application of an action $a$ to a case one can score it's loss $\ell(a)$.
The ASA (Adaptive Scheduling Algorithm) consists of a double loop.
The inner loop iterates over mini batches of cases, referred to as {\em 'rounds'} and collects as many cases in that round so that the total loss is bounded.
The outer loop iterates over such 'rounds' and ensures that the vector $\ell_t\in\R^m$ collecting loss of the various actions $\{a\}$ is initialised properly before starting a new round, 
and that the vector $\pv$ is updated properly after each round.
$\pv$ is a distribution over all possible actions $a$ that can be taken: after a while (when it has learned well), it will peak on the best action $a_\ast$, while in the beginning it is spread evenly over all actions $a$.
In other words, in the beginning the algorithm will {\em explore} options, while an {\em explorative} stance is taken when enough evidence is collected.

\begin{algorithm}
\caption{ASA}
\label{alg.asax}
\begin{algorithmic}
\REQUIRE Initialise $\pv_0$ as $\pv_{0a}=\frac{1}{m}$ for all $a$.
\FOR{$t=1,2, \dots$}
\STATE Initialise $\ell_{ta}=0$ for all $a$.
\WHILE{$\max_a \ell_{ta} \leq 1$}
\STATE (a) Choose action $a$ according to the vector $\pv_t$.
\STATE (b) Add $\ell_{ta} \leftarrow \ell_{ta} + \ell\left(a\right)$ for this $a$ (otherwise $\ell_{ta} \leftarrow \ell_{ta}$).
\ENDWHILE
\STATE Update as
	\[ \pv_{t+1,a} = \frac{1}{N_t}\pv_{t,a}\exp\left( - \gamma_t \ell_{ta}\right)\]
	for all actions $a$. Here $N_t$ is a normalising factor so that $\sum_a \pv_a = 1$.
\ENDFOR
\end{algorithmic}
\end{algorithm}


Now we extend this algorithm to situations 
where each case has an associated state $\xv\in\R^d$.
That is, at any time slot $s$, an action $a$ is taken with the system in state $\xv$, and the loss becomes than $\ell(a,\xv)$.
Again we have a double loop: the inner loop iterates over cases until collected loss exceeds a threshold.
The outer loop then initiates and updates the parameters accordingly.
Now, instead of having the vector $\pv\in\R^m$ as before,  we make $\pv:\R^d\rightarrow\R^m$ a function of the states $\xv\in\R^d$.
Learning then tries to find this functional relationship.
The central quantity is however the {\em risk}, defined here as a vector in $\R^n$ where 
\begin{equation}
	\rv_i = \ell(a) \pv_i(a)
	\label{eq.asax.}
\end{equation}
We maintain at each round $t$ a vector $\rv_t$ of the total risk accumulated in that round.
At round $t$, we let $\rv_{t,i}$ denote the accumulated risk of the $i$th expert.
We then describe a strategy that performs almost as well as 
\begin{equation}
	\min_\ast \sum_{s=1}^t \sum_{j=1}^{n_s} \pv_\ast(\xv_{sj}) \ell\left(a_{sj}\right).
	\label{eq.excess}
\end{equation}
Observe that the strategy minimising this risk would correspond to the maximum likelihood estimate - 
or we want to follow the expert that assigns most probability to the action with the lowest loss. 
Specifically, we will prove that the {\em excess risk} $E_t$ after $t$ rounds is not too large.
The excess risk is defined here as 
\begin{equation}
	E_t  
	= 
	\sum_{s=1}^t \sum_{j=1}^{n_s} \left( \sum_{i=1}^n \alpha_{s-1,i}\pv_i(\xv_{sj}) \ell\left(a_{sj}\right) \right)
	-	\\	 
	\min_\ast \sum_{s=1}^t \sum_{j=1}^{n_s} \pv_\ast(\xv_{sj}) \ell\left(a_{sj}\right),
	\label{eq.excess}
\end{equation}
where $\xv_{sj}$ denotes the states of the $j$th case in the $s$th round, and where
$a_{sj}$ is the action taken at this case.



\begin{algorithm}
\caption{ASA$_{\mbox{x}}$}
\label{alg.asax}
\begin{algorithmic}
\REQUIRE Initialise $\alpha_{0i}=\frac{1}{n}$ for all $i=1, \dots,n$.
\FOR{$t=1,2, \dots$}
\STATE Initialise the total risk $\rv_{ti}=0$ for all $i=1, \dots,n$ (all experts).
\WHILE{$\max_i \rv_{t,i} \leq 1$}
\STATE (a) Measure the state $\xv$ for this case.
\STATE (b) Compute all $n$ experts $\pv_i(\xv)$, each one providing a vector in $\R^m$.
\STATE (c) Form the mixture $\pv=\sum_{i=1}^n \alpha_{t-1,i} \pv_i(\xv) \in\R^m$.
\STATE (d) Choose action $a$ according to the vector $\pv$.
\STATE (e) Score its loss $\ell(a)$ on the case.
\STATE (e) Update as $\rv_{ti} \leftarrow \rv_{ti} + \pv_i(a) \ell\left(a\right)$ for all $i=1, \dots, n$.
\ENDWHILE
\STATE Update as
	\[ \alpha_{t,i} = \frac{1}{N_t}\alpha_{t-1,i}\exp\left( - \gamma_t \rv_{ti}\right)\]
	for all $i=1, \dots, n$. Here $N_t$ is a normalising factor so that $\sum_{i=1}^n \alpha_{t,i} = 1$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

%\input{setup_v2.tex}

\section{General (Naive) Background}

In Bandit Scheduling Optimization \footnote{In classical multi-armed bandit problem formulation, a gambler is at a row of cassino slot machines (in American-English slang, these are called "one-armed bandits") where she has to decide which machines to play at each time, how many times to play in  each machine and in which order to play them.}, one basically has a set of resources where jobs needs to be assigned according to an Object Function (OF).
This OF can be anything, like for example minimizing the average (expected) queue waiting time for submitted jobs.
The task one party (the learner, or player) has to do is to learn the probability distribution of each one of the available resources by interacting (exploring) with the system in a (finite) time interval during an experiment.
This interaction means, for instance, collocating two jobs in a resource. 
Then, after their execution ends, the learner observes the final status of each one of the jobs (often called 'Reward') . 
Metrics and questions can be posed by for example: "what constraints were or were not violated?", "How was the behavior evolution (CPU, memory, I/O, network,... over time) of the resources while both jobs were running together?".
This process can go for \textit{n} jobs in a pool of resources being managed by a specific queue in a Datacenter with a set of constraints, like for example, deadline.

Once enough learning (based on your questions) has been collected, the player starts exploiting the system in order to make better placements (collocation guesses) so a lower ratio of constraints are missed.

In Multi-Armed Bandit Optimization, there are usually two scenarios\footnote{There is a 3rd scenario, Markovian, but the techniques applied in their analysis are very different from what is done in Stochastic and Adversarial settings.}:\\
(i) Stochastic: The Probability Distributions from the resources you are learning about \textbf{does not} change over the time interval of an experiment;\\
(ii) Adversarial: The Probability Distributions from the resources you are learning about \textbf{does} maliciously (not too random) change over the time interval of an experiment, according to what one of the parties is doing;

An instance of a stochastic setting would be if one places two well behaved jobs in a same server for a couple of times and initiate them in the very same configuration for all repetitions.
There is a high probability that in the end the results will be the same.

On the other hand, in an adversarial setting, what happens is that the consequences of placing the very same jobs in the same server in each repetition would be different, since one of the jobs could (hypothetically) 'steal' resources by somehow learning the behavior of the other job in order to adapt to that.
The task of the learner (Job Scheduler) in this case is to try to learn this malicious behavior of the adversarial in order to mitigate the number of constraints missed.

There are different algorithms for giving theoretical bounds to how fast or how much one has to explore in order to fully learn the probability distributions for all resources. In both scenarios.
They differ in complexity of solution, time for convergence and others.

\section{Challenges}

Different extensions to the main scheduling scheme are of direct relevance in practical scenarios.

Server \textit{capacity} (a resource) can be viewed as single dimensional, but in practice it is usually defined as a multivariate function depending on CPU, memory, network, I/O (Input/Output) utilization.
All of these have capacity fluctuations over time, since they may similarly be shared among other datacenter users.
As such, a practical and natural extension to this problem is to generalize its formulation to multi-dimensional cases 
since one-dimensional packing algorithms can be extended to multiple dimensions by vector packing methods \cite{li2014dynamic}.

Additionally, placing one or more jobs together affect their performance as a whole \cite{janus2017slo}.
That means that the actual utilization of capacity of a job depends on the collocated jobs.
For example, cache misses (and the consequent IO operations) might depend on all active jobs.

\section{Case study}
%%%%%%%%%%%%

Consider the setting where a sequence of jobs have to be scheduled so as to achieve the highest overall throughput.
These jobs are interrelated, and a job can only be executed one earlier (associated) jobs are finished.
Those decencies between jobs are specified as a {\em workflow graph}.

Specifically, we want to submit future jobs ahead of time so that previous required 
computations are finished at the time of {\em actual} execution (when the submission has waited long enough in the waiting queue).
That means, we want to submit jobs at times so that the jobs do not need additional waiting for the resource come free.
In case, we would know the waiting times, we can compute explicitly those pre-emptive submission times.
In realistic scenarios however, we do not know their waiting times: instead we have to learn them from past behavior.
In this context, we can use ASA and ASA$_{\mbox{X}}$ so that we can relate performance to an optimal strategy.

Actions here correspond to pre-emptive submission times:
for example $a_1$ can correspond to submitting a new job when we expect previous calculations to be available after another 10s.
The loss can then be taken proportional to the actual time the previous calculations came available.
For example, if the previous calculations where finished only after $14s$, the loss would be proportional to 14s-10s.
On the other hand, if. previous calculations were finished already after 7s, then the loss could be proportional to 10s-7s.
Now let's define $n$ such actions $a_1, a_2, \dots, a_m$, corresponding with a discretisation of the time.
Then we learn a distribution $\pv$ over those $m$ waiting times (and corresponding actions $a$).

In case of ASA$_{\mbox{X}}$, we need to define state information.
It is reasonable to let this state represent the occupation of the equipment on which the jobs are run.
Roughly, if occupation is high, then one can expect waiting times to be long.
Rather than to describe this relation explicitly, we work with different experts.
For example, let the expert $\pv_i(\xv)$ propose how this state is mapped to a distribution of waiting times for this situation.
Conversaly, when occupation is low, then waiting times are more likely to be small.
